Algorithm for Hamilton-Jacobi equations in density space via a generalized Hopf formula

We design fast numerical methods for Hamilton-Jacobi equations in density space (HJD), which arises in optimal transport and mean field games. We overcome the curse-of-infinite-dimensionality nature of HJD by proposing a generalized Hopf formula in density space. The formula transfers optimal control problems in density space, which are constrained minimizations supported on both spatial and time variables, to optimization problems over only spatial variables. This transformation allows us to compute HJD efficiently via multi-level approaches and coordinate descent methods.

==> HF.tex <==

@article{MFG,
  title = {Mean {{Field Games}}: {{Numerical Methods}}},
  volume = {48},
  number = {3},
  journal = {SIAM Journal on Numerical Analysis},
  author = {Achdou, Yves and Capuzzo-Dolcetta, Italo},
  year = {2010},
  pages = {1136-1162}
}

@article{MFG1,
  title = {Mean {{Field Games}}: {{Numerical Methods}} for the {{Planning Problem}}},
  volume = {50},
  number = {1},
  journal = {SIAM Journal on Control and Optimization},
  author = {Achdou, Yves and Camilli, Fabio and Capuzzo-Dolcetta, Italo},
  year = {2012},
  pages = {77-109}
}

@article{MFG2,
  title = {Mean {{Field Games}}: {{Convergence}} of a {{Finite Difference Method}}},
  volume = {51},
  number = {5},
  journal = {SIAM Journal on Numerical Analysis},
  author = {Achdou, Yves and Camilli, Fabio and Capuzzo-Dolcetta, Italo},
  year = {2013},
  pages = {2585-2612}
}

@article{SMFG,
  title = {Two {{Numerical Approaches}} to {{Stationary Mean}}-{{Field Games}}},
  volume = {7},
  number = {4},
  journal = {Dynamic Games and Applications},
  author = {Almulla, Noha and Ferreira, Rita and Gomes, Diogo},
  year = {2017},
  pages = {657-682}
}

@book{Dim1,
  title = {{Adaptive Control Processes: A Guided Tour}},
  author = {Bellman, Richard E},
  year = {2016}
}

@book{Dim2,
  address = {Mineola, N.Y},
  edition = {Dover ed},
  title = {Dynamic Programming},
  publisher = {{Dover Publications}},
  author = {Bellman, Richard},
  year = {2003},
  annote = {Originally published: Princeton, N.J. : Princeton University Press, 1957}
}

@article{PMFG2,
  title = {Stable Solutions in Potential Mean Field Game Systems},
  volume = {25},
  number = {1},
  journal = {Nonlinear Differential Equations and Applications NoDEA},
  author = {Briani, Ariela and Cardaliaguet, Pierre},
  year = {2018}
}

@article{BC1,
  title = {Augmented {{Lagrangian Methods}} for {{Transport Optimization}}, {{Mean Field Games}} and {{Degenerate Elliptic Equations}}},
  volume = {167},
  number = {1},
  journal = {Journal of Optimization Theory and Applications},
  author = {Benamou, Jean-David and Carlier, Guillaume},
  year = {2015},
  pages = {1-26}
}

@article{NN,
  title = {Iterative {{Bregman Projections}} for {{Regularized Transportation Problems}}},
  volume = {37},
  number = {2},
  journal = {SIAM Journal on Scientific Computing},
  author = {Benamou, Jean-David and Carlier, Guillaume and Cuturi, Marco and Nenna, Luca and Peyr{\'e}, Gabriel},
  year = {2015},
  pages = {A1111-A1138}
}

@article{PMFG1,
  archivePrefix = {arXiv},
  eprinttype = {arxiv},
  eprint = {1509.02505},
  primaryClass = {math},
  title = {The Master Equation and the Convergence Problem in Mean Field Games},
  journal = {arXiv:1509.02505 [math]},
  author = {Cardaliaguet, Pierre and Delarue, Fran{\c c}ois and Lasry, Jean-Michel and Lions, Pierre-Louis},
  year = {2015}
}

@article{PAF,
  title = {First {{Order Mean Field Games}} with {{Density Constraints}}: {{Pressure Equals Price}}},
  volume = {54},
  number = {5},
  journal = {SIAM Journal on Control and Optimization},
  author = {Cardaliaguet, Pierre and M{\'e}sz{\'a}ros, Alp{\'a}r R. and Santambrogio, Filippo},
  year = {2016},
  pages = {2672-2709}
}

@article{Hopf_Lax_2,
  title = {Algorithm for {{Overcoming}} the {{Curse}} of {{Dimensionality For Time}}-{{Dependent Non}}-Convex {{Hamilton}}\textendash{}{{Jacobi Equations Arising From Optimal Control}} and {{Differential Games Problems}}},
  volume = {73},
  number = {2-3},
  journal = {Journal of Scientific Computing},
  author = {Chow, Yat Tin and Darbon, J{\'e}r{\^o}me and Osher, Stanley and Yin, Wotao},
  year = {2017},
  pages = {617-643}
}

@article{Hopf_Lax_4,
  archivePrefix = {arXiv},
  eprinttype = {arxiv},
  eprint = {1704.02524},
  primaryClass = {math},
  title = {Algorithm for {{Overcoming}} the {{Curse}} of {{Dimensionality}} for {{State}}-Dependent {{Hamilton}}-{{Jacobi}} Equations},
  journal = {arXiv:1704.02524 [math]},
  author = {Chow, Yat Tin and Darbon, Jerome and Osher, Stanley and Yin, Wotao},
  year = {2017}
}

@article{Hopf_Lax_3,
  title = {Algorithm for {{Overcoming}} the {{Curse}} of {{Dimensionality For Time}}-{{Dependent Non}}-Convex {{Hamilton}}\textendash{}{{Jacobi Equations Arising From Optimal Control}} and {{Differential Games Problems}}},
  volume = {73},
  number = {2-3},
  journal = {Journal of Scientific Computing},
  author = {Chow, Yat Tin and Darbon, J{\'e}r{\^o}me and Osher, Stanley and Yin, Wotao},
  year = {2017},
  pages = {617-643}
}

@article{JO,
  title = {Algorithms for Overcoming the Curse of Dimensionality for Certain {{Hamilton}}\textendash{}{{Jacobi}} Equations Arising in Control Theory and Elsewhere},
  volume = {3},
  number = {1},
  journal = {Research in the Mathematical Sciences},
  author = {Darbon, J{\'e}r{\^o}me and Osher, Stanley},
  year = {2016}
}

@book{Evans,
  address = {Providence, R.I},
  edition = {2nd ed},
  series = {Graduate studies in mathematics},
  title = {Partial Differential Equations},
  number = {v. 19},
  publisher = {{American Mathematical Society}},
  author = {Evans, Lawrence C.},
  year = {2010},
  annote = {PART I. REPRESENTATION FORMULAS FOR SOLUTIONS: Four important linear PDE -- Nonlinear first-order PDE -- Other ways to represent solutions -- PART II. THEORY FOR LINEAR PARTIAL DIFFERENTIAL EQUATIONS: Sobolev spaces -- Second-order elliptic equations -- Linear evolution equations -- PART III. THEORY FOR NONLINEAR PARTIAL DIFFERENTIAL EQUATIONS: The calculus of variations -- Nonvariational techniques -- Hamilton-Jacobi equations -- Systems of conservation laws -- Nonlinear wave equations}
}

@article{WHJB1,
  title = {Existence of a Solution to an Equation Arising from the Theory of {{Mean Field Games}}},
  volume = {259},
  number = {11},
  journal = {Journal of Differential Equations},
  author = {Gangbo, Wilfrid and Swiech, Andrzej},
  year = {2015},
  pages = {6573-6643}
}

@book{WHJB,
  title = {Hamilton-{{Jacobi}} Equations in the {{Wasserstein}} Space},
  author = {Gangbo, Wilfrid and Nguyen, Truyen and Tudorascu, Adrian},
  year = {2008}
}

@incollection{MFGA,
  address = {Berlin, Heidelberg},
  title = {Mean {{Field Games}} and {{Applications}}},
  volume = {2003},
  booktitle = {Paris-{{Princeton Lectures}} on {{Mathematical Finance}} 2010},
  publisher = {{Springer Berlin Heidelberg}},
  author = {Gu{\'e}ant, Olivier and Lasry, Jean-Michel and Lions, Pierre-Louis},
  editor = {Morel, J.-M. and Takens, F. and Teissier, B.},
  collaborator = {Cousin, Areski and Cr{\'e}pey, St{\'e}phane and Gu{\'e}ant, Olivier and Hobson, David and Jeanblanc, Monique and Lasry, Jean-Michel and Laurent, Jean-Paul and Lions, Pierre-Louis and Tankov, Peter},
  year = {2011},
  pages = {205-266}
}

@article{Hopf_forumula,
  title = {Generalized {{Solutions}} of Non-Linear {{Equations}} of {{First Order}}},
  volume = {14},
  number = {6},
  journal = {Journal of Mathematics and Mechanics},
  author = {HOPF, EBERHARD},
  year = {1965},
  pages = {951-973}
}

@article{CAIN,
  title = {Large Population Stochastic Dynamic Games: Closed-Loop {{McKean}}-{{Vlasov}} Systems and the {{Nash}} Certainty Equivalence Principle},
  volume = {6},
  number = {3},
  journal = {Communications in Information \& Systems},
  author = {Huang, Minyi and Malham{\'e}, Roland P. and Caines, Peter E.},
  year = {2006},
  pages = {221-252}
}

@article{sion1,
  title = {Elementary Proof for {{Sion}}'s Minimax Theorem},
  volume = {11},
  number = {1},
  journal = {Kodai Mathematical Journal},
  author = {Komiya, Hidetoshi},
  year = {1988},
  pages = {5-7}
}

@article{Hopf_MFG,
  title = {Mean Field Games},
  volume = {2},
  number = {1},
  journal = {Japanese Journal of Mathematics},
  author = {Lasry, Jean-Michel and Lions, Pierre-Louis},
  year = {2007},
  pages = {229-260}
}

@article{LiFisher,
  title = {Computations of {{Optimal Transport Distance}} with {{Fisher Information Regularization}}},
  journal = {Journal of Scientific Computing},
  author = {Li, Wuchen and Yin, Penghang and Osher, Stanley},
  year = {2017}
}

@article{PMFG,
  title = {Potential {{Games}}},
  volume = {14},
  number = {1},
  journal = {Games and Economic Behavior},
  author = {Monderer, Dov and Shapley, Lloyd S.},
  year = {1996},
  pages = {124-143}
}

@article{rublev,
  title = {Generalized {{Hopf}} Formulas for the Nonautonomous {{Hamilton}}-{{Jacobi}} Equation},
  volume = {11},
  number = {4},
  journal = {Computational Mathematics and Modeling},
  author = {Rublev, I. V.},
  year = {2000},
  pages = {391-400}
}

@article{sion2,
  title = {On General Minimax Theorems.},
  volume = {8},
  number = {1},
  journal = {Pacific Journal of Mathematics},
  author = {Sion, Maurice},
  year = {1958},
  pages = {171-176}
}

@book{vil2008,
  address = {Berlin},
  series = {Grundlehren der mathematischen Wissenschaften},
  title = {Optimal Transport: Old and New},
  number = {338},
  publisher = {{Springer}},
  author = {Villani, C{\'e}dric},
  year = {2009}
}

@article{proofimportant,
  archivePrefix = {arXiv},
  eprinttype = {arxiv},
  eprint = {1711.03314},
  primaryClass = {math},
  title = {Perspectives on Characteristics Based Curse-of-Dimensionality-Free Numerical Approaches for Solving {{Hamilton}}-{{Jacobi}} Equations},
  journal = {arXiv:1711.03314 [math]},
  author = {Yegorov, Ivan and Dower, Peter},
  year = {2017},
  annote = {Comment: 45 pages, 10 figures}
}

@article{Nelson,
  title = {Derivation of the {{Schr{\"o}dinger Equation}} from {{Newtonian Mechanics}}},
  volume = {150},
  number = {4},
  journal = {Physical Review},
  author = {Nelson, Edward},
  year = {1966},
  pages = {1079-1085}
}

@article{Lafferty,
  title = {The Density Manifold and Configuration Space Quantization},
  volume = {305},
  number = {2},
  journal = {Transactions of the American Mathematical Society},
  author = {Lafferty, John D.},
  year = {1988},
  pages = {699-699}
}

@article{Li-SE,
  archivePrefix = {arXiv},
  eprinttype = {arxiv},
  eprint = {1705.07583},
  primaryClass = {math},
  title = {A Discrete {{Schrodinger}} Equation via Optimal Transport on Graphs},
  journal = {arXiv:1705.07583 [math]},
  author = {Chow, Shui-Nee and Li, Wuchen and Zhou, Haomin},
  year = {2017}
}

@article{Li1,
  archivePrefix = {arXiv},
  eprinttype = {arxiv},
  eprint = {1701.04841},
  primaryClass = {math},
  title = {Entropy Dissipation of {{Fokker}}-{{Planck}} Equations on Graphs},
  journal = {arXiv:1701.04841 [math]},
  author = {Chow, Shui-Nee and Li, Wuchen and Zhou, Haomin},
  year = {2017}
}

@article{Li2,
  archivePrefix = {arXiv},
  eprinttype = {arxiv},
  eprint = {1608.02628},
  primaryClass = {math},
  title = {Entropy Dissipation Semi-Discretization Schemes for {{Fokker}}-{{Planck}} Equations},
  journal = {arXiv:1608.02628 [math]},
  author = {Chow, Shui-Nee and Dieci, Luca and Li, Wuchen and Zhou, Haomin},
  year = {2016}
}

@article{LiG,
  archivePrefix = {arXiv},
  eprinttype = {arxiv},
  eprint = {1803.06360},
  primaryClass = {math},
  title = {Geometry of Probability Simplex via Optimal Transport},
  journal = {arXiv:1803.06360 [math]},
  author = {Li, Wuchen},
  year = {2018}
}

@article{Li4,
  archivePrefix = {arXiv},
  eprinttype = {arxiv},
  eprint = {1712.09266},
  primaryClass = {math},
  title = {Geodesic of Minimal Length in the Set of Probability Measures on Graphs},
  journal = {arXiv:1712.09266 [math]},
  author = {Gangbo, Wilfrid and Li, Wuchen and Mou, Chenchen},
  year = {2017},
  annote = {Comment: 31 Pages}
}

@article{Nelson,
  title = {Derivation of the {{Schr{\"o}dinger Equation}} from {{Newtonian Mechanics}}},
  volume = {150},
  number = {4},
  journal = {Physical Review},
  author = {Nelson, Edward},
  year = {1966},
  pages = {1079-1085}
}

@article{BB,
  title = {A Computational Fluid Mechanics Solution to the {{Monge}}-{{Kantorovich}} Mass Transfer Problem},
  volume = {84},
  number = {3},
  journal = {Numerische Mathematik},
  author = {Benamou, Jean-David and Brenier, Yann},
  year = {2000},
  pages = {375-393}
}




==> macros.tex <==
%% packages
% \usepackage{graphicx}
% \usepackage{subfigure}
% \usepackage{amssymb,amsmath,amsthm}
% \usepackage{latexsym,amsfonts,amscd,amsxtra,amstext}
% \usepackage{algorithm,algorithmic}
% \usepackage[usenames,dvipsnames,svgnames,table]{xcolor} %\usepackage[usenames]{color}
% \usepackage{wrapfig}
\usepackage{mathtools}
\mathtoolsset{showonlyrefs}  % show only used numbers. incompatible with cleveref
\usepackage{etextools}
% %\usepackage{url}
% %\usepackage{hyperref}

% %% macros for commenting
% \usepackage[normalem]{ulem} % to use \sout
% \newcommand{\remove}[1]{{\color{Gray}#1}}
% \newcommand{\revise}[1]{{\color{blue}#1}}
% \newcommand{\commwy}[1]{{\color{Brown}(wy: #1)}} % Wotao Yin

%% show key
\usepackage[color,final]{showkeys}
\definecolor{refkey}{gray}{0.8}
\definecolor{labelkey}{gray}{0.8}

\newcommand{\EMD}{{\mathbf{EMD}}}

%% macros for letters

\newcommand{\va}{{\mathbf{a}}}
\newcommand{\vb}{{\mathbf{b}}}
\newcommand{\vc}{{\mathbf{c}}}
\newcommand{\vd}{{\mathbf{d}}}
\newcommand{\ve}{{\mathbf{e}}}
\newcommand{\vf}{{\mathbf{f}}}
\newcommand{\vg}{{\mathbf{g}}}
\newcommand{\vh}{{\mathbf{h}}}
\newcommand{\vi}{{\mathbf{i}}}
\newcommand{\vj}{{\mathbf{j}}}
\newcommand{\vk}{{\mathbf{k}}}
\newcommand{\vl}{{\mathbf{l}}}
\newcommand{\vm}{{\mathbf{m}}}
\newcommand{\vn}{{\mathbf{n}}}
\newcommand{\vo}{{\mathbf{o}}}
\newcommand{\vp}{{\mathbf{p}}}
\newcommand{\vq}{{\mathbf{q}}}
\newcommand{\vr}{{\mathbf{r}}}
\newcommand{\vs}{{\mathbf{s}}}
\newcommand{\vt}{{\mathbf{t}}}
\newcommand{\vu}{{\mathbf{u}}}
\newcommand{\vv}{{\mathbf{v}}}
\newcommand{\vw}{{\mathbf{w}}}
\newcommand{\vx}{{\mathbf{x}}}
\newcommand{\vy}{{\mathbf{y}}}
\newcommand{\vz}{{\mathbf{z}}}

\newcommand{\vA}{{\mathbf{A}}}
\newcommand{\vB}{{\mathbf{B}}}
\newcommand{\vC}{{\mathbf{C}}}
\newcommand{\vD}{{\mathbf{D}}}
\newcommand{\vE}{{\mathbf{E}}}
\newcommand{\vF}{{\mathbf{F}}}
\newcommand{\vG}{{\mathbf{G}}}
\newcommand{\vH}{{\mathbf{H}}}
\newcommand{\vI}{{\mathbf{I}}}
\newcommand{\vJ}{{\mathbf{J}}}
\newcommand{\vK}{{\mathbf{K}}}
\newcommand{\vL}{{\mathbf{L}}}
\newcommand{\vM}{{\mathbf{M}}}
\newcommand{\vN}{{\mathbf{N}}}
\newcommand{\vO}{{\mathbf{O}}}
\newcommand{\vP}{{\mathbf{P}}}
\newcommand{\vQ}{{\mathbf{Q}}}
\newcommand{\vR}{{\mathbf{R}}}
\newcommand{\vS}{{\mathbf{S}}}
\newcommand{\vT}{{\mathbf{T}}}
\newcommand{\vU}{{\mathbf{U}}}
\newcommand{\vV}{{\mathbf{V}}}
\newcommand{\vW}{{\mathbf{W}}}
\newcommand{\vX}{{\mathbf{X}}}
\newcommand{\vY}{{\mathbf{Y}}}
\newcommand{\vZ}{{\mathbf{Z}}}

\newcommand{\ba}{{\boldsymbol {a}}}
\newcommand{\bb}{{\boldsymbol {b}}}
\newcommand{\bc}{{\boldsymbol {c}}}
\newcommand{\bd}{{\boldsymbol {d}}}
\newcommand{\be}{{\boldsymbol {e}}}
\renewcommand{\bf}{{\boldsymbol {f}}}
\newcommand{\bg}{{\boldsymbol {g}}}
\newcommand{\bh}{{\boldsymbol {h}}}
\newcommand{\bi}{{\boldsymbol {i}}}
\newcommand{\bj}{{\boldsymbol {j}}}
\newcommand{\bk}{{\boldsymbol {k}}}
\newcommand{\bl}{{\boldsymbol {l}}}
\newcommand{\bm}{{\boldsymbol {m}}}
\newcommand{\bn}{{\boldsymbol {n}}}
\newcommand{\bo}{{\boldsymbol {o}}}
\newcommand{\bp}{{\boldsymbol {p}}}
\newcommand{\bq}{{\boldsymbol {q}}}
\newcommand{\br}{{\boldsymbol {r}}}
\newcommand{\bs}{{\boldsymbol {s}}}
\newcommand{\bt}{{\boldsymbol {t}}}
\newcommand{\bu}{{\boldsymbol {u}}}
\newcommand{\bv}{{\boldsymbol {v}}}
\newcommand{\bw}{{\boldsymbol {w}}}
\newcommand{\bx}{{\boldsymbol {x}}}
\newcommand{\by}{{\boldsymbol {y}}}
\newcommand{\bz}{{\boldsymbol {z}}}

\newcommand{\bA}{{\boldsymbol {A}}}
\newcommand{\bB}{{\boldsymbol {B}}}
\newcommand{\bC}{{\boldsymbol {C}}}
\newcommand{\bD}{{\boldsymbol {D}}}
\newcommand{\bE}{{\boldsymbol {E}}}
\newcommand{\bF}{{\boldsymbol {F}}}
\newcommand{\bG}{{\boldsymbol {G}}}
\newcommand{\bH}{{\boldsymbol {H}}}
\newcommand{\bI}{{\boldsymbol {I}}}
\newcommand{\bJ}{{\boldsymbol {J}}}
\newcommand{\bK}{{\boldsymbol {K}}}
\newcommand{\bL}{{\boldsymbol {L}}}
\newcommand{\bM}{{\boldsymbol {M}}}
\newcommand{\bN}{{\boldsymbol {N}}}
\newcommand{\bO}{{\boldsymbol {O}}}
\newcommand{\bP}{{\boldsymbol {P}}}
\newcommand{\bQ}{{\boldsymbol {Q}}}
\newcommand{\bR}{{\boldsymbol {R}}}
\newcommand{\bS}{{\boldsymbol {S}}}
\newcommand{\bT}{{\boldsymbol {T}}}
\newcommand{\bU}{{\boldsymbol {U}}}
\newcommand{\bV}{{\boldsymbol {V}}}
\newcommand{\bW}{{\boldsymbol {W}}}
\newcommand{\bX}{{\boldsymbol {X}}}
\newcommand{\bY}{{\boldsymbol {Y}}}
\newcommand{\bZ}{{\boldsymbol {Z}}}

\newcommand{\balpha}{{\boldsymbol {\alpha}}}
\newcommand{\bbeta}{{\boldsymbol {\beta}}}
\newcommand{\bgamma}{{\boldsymbol {\gamma}}}
\newcommand{\blambda}{{\boldsymbol {\lambda}}}
\newcommand{\brho}{{\boldsymbol {\rho}}}

\newcommand{\cA}{{\mathcal{A}}}
\newcommand{\cB}{{\mathcal{B}}}
\newcommand{\cC}{{\mathcal{C}}}
\newcommand{\cD}{{\mathcal{D}}}
\newcommand{\cE}{{\mathcal{E}}}
\newcommand{\cF}{{\mathcal{F}}}
\newcommand{\cG}{{\mathcal{G}}}
\newcommand{\cH}{{\mathcal{H}}}
\newcommand{\cI}{{\mathcal{I}}}
\newcommand{\cJ}{{\mathcal{J}}}
\newcommand{\cK}{{\mathcal{K}}}
\newcommand{\cL}{{\mathcal{L}}}
\newcommand{\cM}{{\mathcal{M}}}
\newcommand{\cN}{{\mathcal{N}}}
\newcommand{\cO}{{\mathcal{O}}}
\newcommand{\cP}{{\mathcal{P}}}
\newcommand{\cQ}{{\mathcal{Q}}}
\newcommand{\cR}{{\mathcal{R}}}
\newcommand{\cS}{{\mathcal{S}}}
\newcommand{\cT}{{\mathcal{T}}}
\newcommand{\cU}{{\mathcal{U}}}
\newcommand{\cV}{{\mathcal{V}}}
\newcommand{\cW}{{\mathcal{W}}}
\newcommand{\cX}{{\mathcal{X}}}
\newcommand{\cY}{{\mathcal{Y}}}
\newcommand{\cZ}{{\mathcal{Z}}}

\newcommand{\ri}{{\mathrm{i}}}
\newcommand{\rr}{{\mathrm{r}}}


%% macros for math notions and operators

\newcommand{\RR}{\mathbb{R}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\ZZ}{\mathbb{Z}}
\renewcommand{\SS}{{\mathbb{S}}}
\newcommand{\SSp}{\mathbb{S}_{+}}
\newcommand{\SSpp}{\mathbb{S}_{++}}
\newcommand{\sign}{\mathrm{sign}}
\newcommand{\vzero}{\mathbf{0}}
\newcommand{\vone}{{\mathbf{1}}}
\newcommand{\Null}{{\mathrm{Null}}}
\newcommand{\dist}{{\mathrm{dist}}}

\newcommand{\op}{{\mathrm{op}}} % subscript for operator norm
\newcommand{\opt}{{\mathrm{opt}}} % subscript for optimal solution
\newcommand{\supp}{{\mathrm{supp}}} % support
\newcommand{\Prob}{{\mathrm{Prob}}} % probability
\newcommand{\Diag}{{\mathrm{Diag}}} % vector -> diagonal matrix
\newcommand{\diag}{{\mathrm{diag}}} % matrix diagonal -> vector
\newcommand{\dom}{{\mathrm{dom}}} % domain
\newcommand{\grad}{{\nabla}}    % gradient
\newcommand{\tr}{{\mathrm{tr}}} % trace
\newcommand{\TV}{{\mathrm{TV}}} % total variation
\newcommand{\Proj}{{\mathrm{Proj}}}
\newcommand{\prj}{{\mathbf{proj}}}
\newcommand{\prox}{{\mathbf{prox}}}
\DeclareMathOperator{\shrink}{shrink} % shrinkage
\DeclareMathOperator*{\argmin}{arg\,min} % argmin
\DeclareMathOperator*{\argmax}{arg\,max} % argmax
\DeclareMathOperator*{\mini}{minimize}
\DeclareMathOperator*{\maxi}{maximize}
\newcommand{\st}{{\quad\text{s.t.}~}} % s.t.
\newcommand{\St}{{\text{subject to}~}} % s.t.

\newcommand{\TDRS}{T_{\mathrm{DRS}}}
\newcommand{\TPRS}{T_{\mathrm{PRS}}}
\newcommand{\TFBS}{T_{\mathrm{FBS}}}

\DeclareMathOperator*{\Min}{minimize}
\DeclareMathOperator*{\Max}{maximize}
\DeclareMathOperator*{\Fix}{Fix}
\DeclareMathOperator*{\zer}{zer}
\DeclarePairedDelimiter{\dotp}{\langle}{\rangle}


%% macros for environments math equations

\newcommand{\MyFigure}[1]{../fig/#1}

\newcommand{\bdm}{\begin{displaymath}}
\newcommand{\edm}{\end{displaymath}}

\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}

\newcommand{\bfl}{\begin{flushleft}}
\newcommand{\efl}{\end{flushleft}}

\newcommand{\beqn}{\begin{eqnarray}}
\newcommand{\eeqn}{\end{eqnarray}}

\newcommand{\beqs}{\begin{align*}} % no equation numbers
\newcommand{\eeqs}{\end{align*}}  % no equation numbers


\newcommand{\bld}[1]{\boldsymbol{#1}}
\newcommand{\mbfa}{\mathbf{A}}
\newcommand{\mbfb}{\mathbf{B}}
\newcommand{\mbfc}{\mathbf{C}}
\newcommand{\mbfd}{\mathbf{D}}
\newcommand{\mbfg}{\mathbf{G}}
\newcommand{\mbfi}{\mathbf{I}}
\newcommand{\mbfm}{\mathbf{M}}
\newcommand{\mbfs}{\mathbf{S}}
\newcommand{\mbfx}{\mathbf{X}}
\newcommand{\mbfy}{\mathbf{Y}}

\newcommand{\mbc}{\mathbb{C}}
\newcommand{\mbr}{\mathbb{R}}

\newcommand{\mca}{\mathcal{A}}
\newcommand{\mcb}{\mathcal{B}}
\newcommand{\mcc}{\mathcal{C}}
\newcommand{\mcd}{\mathcal{D}}
\newcommand{\mcf}{\mathcal{F}}
\newcommand{\mcg}{\mathcal{G}}
\newcommand{\mci}{\mathcal{I}}
\newcommand{\mcj}{\mathcal{J}}
\newcommand{\mcl}{\mathcal{L}}
\newcommand{\mcm}{\mathcal{M}}
\newcommand{\mcn}{\mathcal{N}}
\newcommand{\mcp}{\mathcal{P}}
\newcommand{\mcq}{\mathcal{Q}}
\newcommand{\mcs}{\mathcal{S}}
\newcommand{\mcu}{\mathcal{U}}
\newcommand{\mcv}{\mathcal{V}}
\newcommand{\mcx}{\mathcal{X}}
\newcommand{\mcy}{\mathcal{Y}}

\newcommand{\bfx}{\mathbf{x}}
\newcommand{\bfa}{\mathbf{a}}
\newcommand{\bfb}{\mathbf{b}}
\newcommand{\bfc}{\mathbf{ c}}
\newcommand{\bfd}{\mathbf{ d}}
\newcommand{\bfe}{\mathbf{ e}}
\newcommand{\bfg}{\mathbf{g}}
\newcommand{\bfp}{\mathbf{p}}
\newcommand{\bfs}{\mathbf{s}}
\newcommand{\bfy}{\mathbf{y}}
\newcommand{\bfz}{\mathbf{z}}
\newcommand{\bfu}{\mathbf{u}}
\newcommand{\bfv}{\mathbf{v}}
\newcommand{\bfw}{\mathbf{w}}

% \makeatletter
% \newcommand{\Spvek}[2][r]{%
%   \gdef\@VORNE{1}
%   \left(\hskip-\arraycolsep%
%     \begin{array}{#1}\vekSp@lten{#2}\end{array}%
%   \hskip-\arraycolsep\right)}

% \def\vekSp@lten#1{\xvekSp@lten#1;vekL@stLine;}
% \def\vekL@stLine{vekL@stLine}
% \def\xvekSp@lten#1;{\def\temp{#1}%
%   \ifx\temp\vekL@stLine
%   \else
%     \ifnum\@VORNE=1\gdef\@VORNE{0}
%     \else\@arraycr\fi%
%     #1%
%     \expandafter\xvekSp@lten
%   \fi}
% \makeatother

%% macros for theorem-like environments

%\newtheorem{theorem}{Theorem}
%\newtheorem{assumption}{Assumption}
%\newtheorem{definition}{Definition}
%\newtheorem{corollary}{Corollary}
%\newtheorem{remark}{Remark}
%\newtheorem{lemma}{Lemma}
%\newtheorem{proof}{Proof}
%\newtheorem{proposition}{Proposition}
%\newtheorem{example}{Example}

%\newtheorem{example}[remark]{Example}



